EP-HDC: Hyperdimensional Computing with Encrypted Parameters for High-Throughput Privacy-Preserving Inference

While homomorphic encryption (HE) provides strong privacy protection, its high computational cost has restricted its application to simple tasks. Recently, hyperdimensional computing (HDC) applied to HE has shown promising performance for privacy-preserving machine learning (PPML). However, when applied to more realistic scenarios such as batch inference, the HDC-based HE has still very high compute time as well as high encryption and data transmission overheads. To address this problem, we propose HDC with encrypted parameters (EP-HDC), which is a novel PPML approach featuring client-side HE, i.e., inference is performed on a client using a homomorphically encrypted model. Our EP-HDC can effectively mitigate the encryption and data transmission overhead, as well as providing high scalability with many clients while providing strong protection for user data and model parameters. In addition to application examples for our client-side PPML, we also present design space exploration involving quantization, architecture, and HE-related parameters. Our experimental results using the BFV scheme and the Face/Emotion datasets demonstrate that our method can improve throughput and latency of batch inference by orders of magnitude over previous PPML methods (36.52~1068x and 6.45~733x, respectively) with less than 1% accuracy degradation.

==> save-dac/body.tex <==
% Q: However, previous HE-HDC approaches have encountered challenges related to accuracy and throughput. This paper introduces an enhanced HDC-based PPML approach tailored for real-time object detection on commodity hardware. Key advancements

% Q: however its accuracy is limited, -> can we do this?
% accuracy isn't really improved

\begin{abstract}
While homomorphic encryption (HE) provides robust privacy protection, its high computational demands have restricted its application to simple tasks. Recently, hyperdimensional computing (HDC) applied to HE has shown promise in significantly enhancing performance compared to prior privacy-preserving machine learning (PPML) techniques. \red{However, previous HE-HDC approaches have encountered challenges related to accuracy and throughput.
This paper introduces an enhanced HDC-based PPML approach tailored for real-time object detection on commodity hardware. Key advancements} include: (i) leveraging client-side HE to mitigate encryption and data transmission overhead, (ii) employing HE-aware quantization, and (iii) optimizing parameters through systematic exploration of the design space. Our experimental findings indicate that our method surpasses previous PPML techniques by a factor of $55.7\sim 2027\times$ in throughput and $6.94\sim 787\times$ in latency. Consequently, it enables homomorphically encrypted real-time object detection with remarkable efficiency.
%  Despite its robust privacy protection, homomorphic encryption (HE) imposes excessive computational burdens, limiting its applicability to simplistic tasks only. Recently, hyperdimensional computing (HDC) evaluated on HE has been shown to offer a substantial performance boost compared to previous privacy-preserving machine learning (PPML) methods. However, the prior HE-HDC approach suffers from accuracy and throughput issues. This paper presents an improved HDC-based PPML method for real-time object detection on commodity hardware. Key features include (i) using client-side HE to reduce encryption and data transmission overhead, (ii) HE scheme aware quantization and (iii) optimizing parameters through systematic design space exploration. Our experimental results demonstrate that our method outperforms previous PPML methods by $55.7\sim 2027\times$ in throughput and $6.94\sim 787\times$ in latency, and can be fast enough to enable homomorphically-encrypted real-time object detection. 
\end{abstract}
%Z(i) integrating a HOG feature extractor for enhanced image classification accuracy, 
%\keywords{Artificial Neural Networks (ANNs), Deep Convolutional Neural Networks (DCNNs), Stochastic Computing (SC)}

\maketitle

\section{Introduction}
As artificial intelligence gains popularity, there is an increasing demand to ensure privacy of user data. Homomorphic Encryption (HE) offers a robust solution by enabling arithmetic operations on ciphertext without ever revealing the encryption key or plaintext. However, previous applications of HE-based privacy preserving machine learning (PPML) \cite{cryptonets:icml16,lola} have been restricted to very small networks and simplistic tasks. When dealing with more complex applications where privacy protection actually makes sense (e.g., real-time face detection and authentication), the computational demands of HE can pose significant barriers.

Recently, a promising alternative based on hyperdimensional computing (HDC) has emerged as a way to achieve faster HE-based PPML. HDC relies on large vectors and a few simple mathematical operations, which has helped \emph{HE-HDC}, or HDC evaluated on HE, to be much more performant than Deep Neural Network (DNN)-based PPML approaches \cite{hehdc}.  Nevertheless, the previous HE-HDC method suffers from two critical shortcomings: diminished inference accuracy and insufficient throughput for more complex applications such as real-time object detection.

In this paper, we present a vastly improved HDC-based PPML framework dubbed \emph{HeroHD}, which improves inference accuracy, latency, throughput, and network communication overhead over the previous HDC-based PPMLs.
Whereas previous PPMLs, whether DNN-based and HDC-based, target simplistic tasks only such as image classification, HeroHD is the first PPML framework that is capable of achieving real-time object detection performance on commodity hardware. 
The key features of HeroHD, which are also our contributions, include: (i) client-side HE to reduce encryption and data transmission overhead, (ii) integer HE-aware quantization, and (iii) a systematic design space exploration that co-optimizes quantization, HDC model hyperparameters, and HE parameters together.

It is worth noting that client-side HE for PPML is quite a novel concept. One of the surprising results of client-side HE is that it can greatly reduce client runtime despite the fact that some work (similarity search) is actually migrated to client. 
We also provide security analysis of client-side HE.

%\jlnote{is (i) above also our contribution, because it seems not? If so, we need to state it explicitly. Also (iii) may need some defense.}

Our experimental results demonstrate that HeroHD can achieve $615\times$ higher throughput compared to the previous SoTA HDC-based PPML (HE-HDC) \cite{hehdc} and outperforms DNN-based methods with $55.7 \sim 2027\times$ higher throughput and a latency improvement of $6.94 \sim 787\times$ at comparable accuracy.

\ignore{Contributions
- Batched HDC Inference using HE (-> previous work)

- HDC optimization (좀 novelty가 약함)

- Client side HE approach 
  - Optimization for Real Time HE OD (incl. Parameter Optimization)
- Quantization
}

\ignore{In this paper we make the following contributions.
First, motivated by our analyis  on data size and compute complexity, we propose client-side HE approach for HDC-based PPML.  While applicability amy depend on application requirement, but it assumes a similar threat model as previous PPML, but can have  much improved latency and throughtput.
Second, naive approach can be very slow, but we optimize crypto parameters 
so that HE-based OD can be run real time on a commodity CPU.
Third, we perform quantization to further optimize the performance of HE-based 

Client can perform image processing on the raw message, which is far more efficient than on ciphertext or even plaintext.
Client does not need to send large data but model size.


(Transpose this table to save space)
         message   model size
IC-CNN    small     large
IC-HD     small     small
OD-CNN    small     larger
OD-HD     large     small
}

\begin{table}[t]
  \caption{List of symbols}
  \label{t:sym}
  \centering
  \begin{tabular}{c|l}
    \toprule
    Symbol & \multicolumn{1}{c}{Description} \\
    \midrule
    $N$ & Polynomial degree for plaintext/ciphertext (a power of 2) \\
    %\cmidrule{2-3}
    %    $\log_2 t$ & Bit-length of the message inside the ciphertext \\
    $\log_2 t$ & Bit-length of the message (each element's in case of a vector) \\
    %\cmidrule{2-3}
    $D$ & Hypervector dimension (typ. 4K$\sim$10K) \\
    %  $\vec{\mathcal{C}}$ & Class hypervector (of dimension $D$) \\
    %  $\vec{\mathcal{H}}_q$ & Query hypervector (of dimension $D$) \\
    $k$ & Number of class hypervectors \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Related Work}
\subsubsection*{Privacy-Preserving Machine Learning}
%FHE-DiNN \cite{she:nips18} is a framework for homomorphic evaluation of neural networks, in which each neuron's output is refreshed through bootstrapping.
%Juvekar \etal \cite{gazelle} develop Gazelle, a scalable and low-latency system for secure neural network inference, which contains a homomorphic encryption library, homomorphic linear algebra kernels, and optimized encryption switching protocols.
Dowlin \etal \cite{cryptonets:icml16} present \emph{CryptoNets}, neural networks that can be applied to encrypted data to make accurate predictions while maintaining data privacy and security.
\emph{Faster CryptoNets} \cite{chou2018faster} accelerates the homomorphic evaluation by employing a pruning and quantization approach that leverages sparse representations.
Low-Latency CryptoNets \cite{lola} changes data representation throughout computation in a novel way to reduce latency while maintaining accuracy and security. 
%Boemer \etal \cite{boemer2019ngraphhe} introduce nGraph-HE, a graph compiler, which enables the deployment of trained models with popular DL frameworks while simply treating HE as another hardware target. 
%Hesamifard \etal \cite{ehsan2019} design a privacy-preserving classification for convolutional neural networks (CNNs) over encrypted data, which replaces commonly used activation functions in CNNs with low-degree polynomials.
Hesamifard \etal \cite{ehsan2019} replace nonlinear activation functions with low-degree polynomials.
%Benaissa \etal \cite{benaissa2021tenseal} present TenSEAL, a flexible open-source library, for doing encrypted tensor computation using homomorphic encryption.
Lee \etal\cite{mp-fhe-cnn} propose a faster multiplexed parallel convolution algorithm to reduce the number of required rotations using full ciphertext slots, in addition to a multiplexed packing method, which packs data of multiple channels into one ciphertext, reducing the runtime overhead of bootstrapping.
%Liu \etal \cite{trusted-dnn} propose Trusted-DNN, an overall DNN model protection strategy based on TrustZone and encryption algorithms oriented to the security issues of embedded devices.
Recently, an HDC-based approach \emph{HE-HDC} \cite{hehdc} was proposed, which can be implemented using HE-friendly operations only, thus improving the latency of PPML considerably.

\subsubsection*{Hyperdimensional Computing}
NeuralHD \cite{neuralhd} is the first HDC algorithm with a dynamic and regenerative encoder for adaptive learning, and can enhance learning capability and robustness by identifying insignificant dimensions and regenerating those dimensions. 
%ManiHD \cite{zou2021manihd} provides trainable encoding that considers non-linear interactions between features. 
VoiceHD \cite{voicehd} is an efficient and hardware-friendly speech recognition technique using HD computing, which maps preprocessed voice signals in the frequency domain to hypervectors and combines them to compute class hypervectors. 
AdaptHD \cite{adapthd} is an adaptive retraining method for HD computing, which introduces the idea of learning rate to HD computing and proposes a hybrid approach to update the learning rate considering both iteration and data dependency.
%OnlineHD \cite{onlinehd} identifies common patterns in each class hypervector and eliminates model saturation. 
Instead of simple hypervector averaging, OnlineHD \cite{onlinehd} updates a model differently depending on the model prediction result, enabling iterative training and potentially boosting performance of HDC models.
%Kim \etal \cite{cascadehd} propose CascadeHD, an efficient many-class classification learning framework, which considers the inter-dependency of different classes by revising the iterative hypervector fine-tuning procedure and identifies confusing classes while learning a hierarchical inference structure by a meta-learning algorithm.
%Prive-HD \cite{privhd} considers HD computing from a privacy perspective. HD computing has no privacy due to its reversible computation. Prive-HD realizes a differentially private HD model as well as blurs the information sent for cloud-hosted inference by quantization and pruning. 


\section{Preliminary}
%Here we discuss the preliminaries related to hyperdimensional computing and homomorphic encryption. For the ease of understanding,
%\tabref{t:sym} lists the symbols frequently used in this paper.





\subsection{Hyperdimensional Computing}

%Hyperdimensional computing (HDC) is an alternative machine learning paradigm developed based on the observation that the human brain operates on high-dimensional data \cite{kanerva2009hyperdimensional}.
HDC is a brain-inspired machine learning paradigm based on high-dimensional vector representation called \emph{hypervector} \cite{kanerva2009hyperdimensional}.
%The fundamental unit of computation in HDC is , which refers to a high-dimensional vector used to represent and manipulate complex data patterns and information.
The HDC approach has many advantages over DNNs including more efficient training (not based on back-propagation), higher robustness against noise, and superior generalization performance \cite{rahimi2016hyperdimensional, 7838428, thomas2021theoretical, neuralhd}. However, its ability to extract features from complex data (e.g., image/video) is limited. Consequently a pre-processing procedure such as feature extraction is needed to extract useful information from raw data.
%\figref{hdc-od} illustrates an overview of our HDC-based object detection framework.

%\noindent\textbf{Feature Extraction:} 
%There are various existing feature extraction mechanisms for object detection such as convolution, HAAR-like feature extraction, and Histogram of oriented Gradients (HOG). Here we briefly explain HOG since we use it in our experiments.

%\noindent\textbf{HOG:}
%Histogram of oriented Gradients (HOG) is a widely used feature extraction technique in computer vision and image processing. %It is particularly effective in capturing the shape and texture information of objects within images. 
%HOG operates by dividing an image into small regions, computing histograms of gradient orientations within these regions, and then concatenating these histograms to form a feature vector.
%\jlnote{this doesn't belong to HDC; let's move this to a different place}

\noindent\textbf{HDC Encoding:}
The goal of HDC encoding is to discover a well-defined hypervector representation for input data. Though there are multiple existing encoding schemes \cite{neuralhd, voicehd, adapthd, onlinehd}, they all satisfy the common-sense principle: different data points in the original space should have orthogonal hypervectors in the HDC space. For example, random projection encoding~\cite{onlinehd} transforms a flattened image vector into hypervectors by multiplying a random base hypervector. 
%$\vec{X}_q$ of length $K$ into a hypervector $\vec{\mathcal{H}}_q$ of length $D$ as follows: 
%$\vec{\mathcal{H}}_q = \cos(B \vec{X}_q + \vec{b}) \otimes \sin(B \vec{X}_q)$
%, where $B$ is a $(D \times K)$-sized matrix, whose columns are random hence orthogonal %\emph{base hypervectors} drawn from a standard normal distribution; $\vec{b}$ is another random base hypervector of length $D$ drawn from a uniform distribution in $[0, 2 \pi]$; and $\otimes$ is element-wise multiplication.

\noindent\textbf{Single-pass Training:}
Once input hypervectors are generated, the hypervectors
belonging to the same class are averaged to obtain a class hypervector. 
%Assuming there are $J$ inputs having label $l$: $\vec{\mathcal{C}^l} = \sum^{J}_{j} \vec{\mathcal{H}}_{qj}^l$.
%A class hypervector contains the generalized information of each class by linearly combining procedures, which does not require error back-propagation.

\noindent\textbf{Inference:}
The classification of a query data is performed by first encoding the query data to a query hypervector $\vec{\mathcal{H}}_q$, and then computing the similarity of $\vec{\mathcal{H}}_q$ with each class hypervector. %$\vec{\mathcal{C}^l}$. 
The class with the highest similarity score is returned as the classification result. For the similarity measure, the cosine similarity is widely used.
%Query data gets the label with the highest similarity. 
%For the similarity measure ($\delta$), cosine similarity is typically used:
    %$\delta(\vec{\mathcal{H}}_q,\vec{\mathcal{C}^l}) = \frac{\vec{\mathcal{H}}_q^\intercal \cdot \vec{\mathcal{C}^l}}{\Vert \vec{\mathcal{H}}_q \Vert_2 \cdot \Vert \vec{\mathcal{C}^l} \Vert_2 }$, where $\Vert \cdot \Vert_2$ represents the $L_2$ norm.

\noindent\textbf{Iterative Training (Retraining):}
Due to the poor classification accuracy of single-pass training, using an iterative training method is suggested, which discards mispredicted queries from mispredicted classes and adds them to correct classes \cite{onlinehd}. %Given a query hypervector $\vec{\mathcal{H}_q}$ with the correct label $l$ and the mispredicted label $m$, the class hypervectors are updated as follows ($\eta$ is learning rate):
%$\vec{\mathcal{C}^l} = \vec{\mathcal{C}^l} + \eta (1-\delta(\vec{\mathcal{H}}_q, \, \vec{\mathcal{C}^l})) \vec{\mathcal{H}}_q$, 
%$\vec{\mathcal{C}^m} = \vec{\mathcal{C}^m} - \eta (1-\delta(\vec{\mathcal{H}}_q, \, \vec{\mathcal{C}^m}))  \vec{\mathcal{H}}_q$

\subsection{Homomorphic Encryption}
%The three schemes differ in how the message is encoded into a pair of polynomials. %(see \tabref{t:scheme_comp}).
%CKKS is the most widely used scheme in HE-based PPML thanks to its support for fixed-point message vectors; however, the dimension of the message vector is half of others.
%\blue{On the other hand, BGV and BFV schemes support integer arithmetic and can be faster than CKKS when the number of homomorphic multiplications is low \cite{fhebench}.} \todo{move to another section}

%When a vector is encoded as a message in an HE scheme,
%\red{\em The following sentence needs to be revised.}
Homomorphic encryption allows arithmetic operations such as multiplication and addition to be evaluated on encrypted data. The majority of HE schemes are based on the ring learning with errors  (LWE) problem, where the underlying operations are performed over polynomials of degree $N$. In HE, a message is first \emph{encoded} into a plaintext $(c_0,c_1)$, which is a pair of polynomials of degree $N$, and then the plaintext is \emph{encrypted} into a ciphertext using a given secret key. Homomorphic operations can be performed between two ciphertexts or between a ciphertext and a plaintext, resulting in a ciphertext encrypted with the same secret key.

HE schemes such as CKKS \cite{ckks}, BGV \cite{bgv}, and BFV \cite{bfv} can encode a vector of $N$ integers into a single plaintext ($N/2$ fixed-point for CKKS) which is referred to as \emph{packing}. When packing is used, homomorphic multiplication and addition are evaluated as element-wise operations between two message vectors (analogous to SIMD). However, the individual elements of a ciphertext message vector cannot be accessed unless decrypted. The only way to change the position of elements inside the message vector is by homomorphic rotation. %, where the order of elements inside the message vector is shifted by a arbitrary value.
Homomorphic rotation has a much longer latency than addition and multiplication, and therefore should be avoided as much as possible to achieve high performance.
%\blue{When homomorphically evaluating computation over high dimensional data such as matrix multiplication it is crucial to choose the representation of matrices and tensors into ciphertexts that minimizes the number of homomorphic rotations.} \todo{could be moved to later section, or removed}
\ignore{
\begin{table}[t]
  \centering
  \caption{Comparison between different HE schemes}
  \label{t:scheme_comp}
  \begin{tabular}{c|ccc}
      \toprule
                 & CKKS                & BGV     & BFV     \\
                     \midrule
Arithmetic       & fixed-point complex & integer & integer \\
\# of SIMD slots & $N/2$                 & $N$       & $N$      \\
    \bottomrule
    %\multicolumn{2}{l}{\emph{Note.}~ $N$ refers to the polynomial degree.} \\
\end{tabular}
\end{table}}

%In order to maintain security while ensuring the correctness of computation, homomorphic encryption adds noise into ciphertexts. Homomorphic operations gradually increase the noise level inside a ciphertext. The coefficients of each polynomial in a ciphertext has a fixed precision, the ciphertext modulo's bit-length, $\log_2 q$, which is determined by the security level. The ciphertext precision can be increased by sacrificing security or increasing the ciphertext polynomial degree.




\subsection{Threat Model}
This work assumes the common threat model suggested in previous PPML works \cite{cryptonets:icml16,lola,hehdc}. This model involves two parties, the client and the server, with the server providing ML-based object detection as a service. The client does not want to expose its original image to the server, while the server prefers not to reveal the ML model (i.e., the class hypervectors) to the client. Similar to two-party computation (2PC) approaches \cite{reagen2021cheetah,gazelle}, we assume that the client is honest in performing its computation but curious about the ML model.


\begin{figure}
    \centering
    \myincludegraphics[width=\linewidth]{hdc-od}{HDC-based object detection framework overview.}
    %\label{fig_hdc-od}
\end{figure}

\section{Application: HDC-based Object Detection}
\label{section_hdod}
%\todonum[]{Chenghao, can you help me write this?}
%\todonum[]{JW, I will try to revise this so that including HOG is on of our contributions}
%Although HDC is efficient in computing with abstract information, the main drawback is in  extracting features from complex data such as images and videos. %It is necessary to rely on a feature extractor, such as HOG, to extract useful information from raw data. 
Though HDC-based approach is more affordable than DNN-based approach when evaluated on HE, the poor classification accuracy of HDC limits the use of HDC to simplistic tasks only. Here, in order to overcome the poor accuracy of HDC models, we propose to attach a HOG feature extractor to extract information from raw images.
%Additional benefit in using the HOG feature extractor is that the size of the HOG feature map is smaller than that of the raw image, which reduces the size of the random matrix in the HDC encoder and the HDC encoding latency. 
%We show the accuracy and latency improvement from using the HOG feature extractor in\secref{subsection_hdc-opt}.
Illustrated in \figref{hdc-od}, our HDC-based object detection flow consists of three steps:
\begin{enumerate}
    \item Starting with an image frame, we employ a sliding window approach to generate a set of overlapping windows.
    \item For each of these windows, we utilize a HOG feature extractor to create a corresponding feature map.
    \item The HDC model takes the HOG feature maps and determines if an object is within each window.
\end{enumerate}

In Step 1, a part of the image is taken as an image-window where the window slides through the image frame left to right, row by row. This sliding window technique generates a set of overlapping image-windows to be processed next.
In Step 2, we feed these image-windows to a HOG feature extractor, which computes a feature map for each image-window.
In Step 3, the generated feature maps are fed to the HDC model, which encodes every feature map into a query hypervector, and calculates the cosine similarity score between query hypervectors and class hypervectors. Based on the similarity score the model determines whether there is an object inside a window as well as the class of an object using multiple class hypervectors. For the HDC model, we employ the encoder and the iterative training method proposed in \cite{onlinehd}.
%Here we simplify the cosine similarity calculation to the matrix multiplication between the query hypervector and the normalized class hypervectors as in our previous work \cite{hehdc}.% Furthermore, we quantize the query hypervector and the normalized class hypervectors to non-negative integers during the inference. More details about quantization are explained in Section \ref{subsection_quant}. Finally, the feature map gets the label of the class with the highest similarity score and determines if the window has an object we interest.


\begin{figure}  
  \myincludegraphics[width=\linewidth]{lat_breakdown}{Breakdown of HE runtime in server-side setting of \figref{overview}.}
\end{figure}

\begin{figure*}
  \myincludegraphics[width=\linewidth]{overview}{Server-side HE vs.\ our proposed client-side HE (HeroHD) for object detection. HV stands for hypervector.}
\end{figure*}

\section{HeroHD}

%\subsection{Overview}

%\figref{overview} illustrates the overall procedure of HeroHD, which has three novel features: (i) the client-side HE computation, intended to reduce overall runtime and network transmission overhead; (ii) the HE/HDC co-optimization design flow for optimizing both HDC model and HE parameters; and (iii) the BGV/BFV-aware quantization scheme to maintain high accuracy under extremely low HE precision. These three features are closely interrelated, necessitating a holistic approach to co-optimize the entire system. Our goal is to maintain both low latency and high throughput for real-time object detection on HE.
%\figref{overview} illustrates the overall flow of HeroHD, which has three novel features: (i) the HDC component, aimed at achieving high accuracy in object detection; (ii) the homomoprhic computation mapping for batched HDC inference; and (iii) client-side HE computation, intended to reduce overall runtime and network transmission overhead. We show that these design components are closely interrelated, necessitating a holistic approach to co-optimize the entire system. Our goal is to maintain both low latency and high throughput for real-time object detection on HE.

HeroHD is a \textit{client-side HE computation framework} designed to reduce overall runtime and network transmission overhead for \textit{batched HDC inference}. 
We first motivate the need for client-side HE computation for our target application, then present our HeroHD and our optimizations for HeroHD. 
%batched these design components are closely interrelated, necessitating a holistic approach to co-optimize the entire system. 
%Our goal is to maintain both low latency and high throughput for real-time object detection on HE.

\subsection{Client-side HE Computation}
\subsubsection{Server-side HE}
The left side of \figref{overview} illustrates the traditional server-side HE when used for object detection.
Starting from a raw image frame, the client applies sliding window and generates multiple query hypervectors. The query hypervectors are then encrypted into ciphertexts and sent to the server. The server homomorphically computes the cosine similarity search and send the resulting similarity scores to the client, where the client decrypts the results. 
Due to the heavy computation cost of HE operations, most HE-based PPML approaches assume a setting where HE arithmetic operations are performed on the server and the client only performs ciphertext encryption. However, ciphertext encryption has the longest latency among all HE operations, up to $N < 2^{13}$ \cite{hehdc}, and therefore cannot be ignored in latency-critical applications. Moreover, object detection requires many rounds of ciphertext encryption resulting in large client runtime as well as large message size, leading to increased communication overhead. %On top of such traditional server-side HE computation setting, HeroHD has to encrypt thousands of hypervectors for a single image frame which dominates the total runtime. 

%Surprisingly, we observe that the na\"ive implementation of HeroHD where the cosine similarity search happens one the server the client has more computations than the server due to the large ciphertext encryption overhead.

\figref{lat_breakdown} presents the total HE runtime breakdown of traditional server-side HE in various settings. Here, the server has to encode class hypervectors into plaintexts and perform the cosine similarity search homomorphically whereas the client should encrypt input image frames into ciphertexts. 
This ciphertext encryption overhead can be resolved by computing the cosine similarity search homomorphically on the client, not on the server. 

\subsubsection{Client-side HE}
The right side of \figref{overview} illustrates our client-side HE, of which the main highlights are the following:
\begin{itemize}
    \item Instead of encrypting query HVs into ciphertext, the class HVs are encrypted, which needs to be performed and sent only once beforehand.% Client-side HE eliminates the need for ciphertext encryption by 
    \item Homomorphic similarity search is performed on the client instead of the server. Though this (i.e., client-side similarity search) increases client runtime, it is far outweighed by runtime saving due to the elimination of ciphertext encryption.
    \item Reduced communication: instead of client sending a set of encrypted query HVs for every image, client now needs to send only the encrypted cosine similarity scores.% which is $D$ times less in size.
\end{itemize}
%After client performs the similarity search, the ciphertexts containing the similarity scores are sent to the server where the server decrypts and send the detection results back to the client. 

\subsubsection{Security Analysis of HeroHD}
To keep model secrecy from the client, the class hypervectors are encrypted into ciphertexts where the query hypervectors remain in the plaintext domain. 
%Unlike query hypervectors which has to be generated and encrypted runtime, the class hypervector only needs to be encrypted once from the server before deployed to the client therefore eliminating ciphertext encryption. 
This client-side approach is valid in the original threat model, since the class hypervectors are not exposed to the users and the user's private data is never sent to the server. We note that the inference result (in our case, object detection result) is revealed to the server, which is not an issue in applications such as face-based authentication (assuming that the HE server is also the authentication server), but could be an issue depending on the application scenario.  On the other hand, the revelation of inference result to the server is not a violation of the threat model, and it is hard for the server to recover the original data from the similarity score alone.

Prive-HD \cite{privhd} argues that even if query HVs are revealed, raw image can be protected by employing quantization and pruning of query HVs.  Our case is significantly more challenging to break (i.e., recover the raw image), since we only reveal the similarity score, not query HVs. Further, we already send quantized versions of similarity scores to the server by virtue of using an integer HE scheme (see \secref{subsection_quant}).

%the input image can be restored from query hy by 
%The difference with the privacy of server-side HE is that the result is exposed to the server which may lead to 


\ignore{
\begin{figure}
  \myincludegraphics[width=\linewidth]{he-hdc}{Cosine similarity search in HE-HDC \cite{} between a single query hypervector of $D=4$ and two class hypervectors. A single ciphertext of $N=4$ is used to encrypt the query hypervector and two plaintexts are used.}
\end{figure}


\begin{figure}  
  \myincludegraphics[width=\linewidth]{hero-hdc}{Cosine similarity search in our HeroHD between two query hepervectors and two class hypervectors of $D=4$. The ciphertext polynomial degree is equal to the batch size of query hypervectors and four plaintext are used to encode hypervectors of $D=4$. Gray color indicates plaintext formats whereas the colored parts with similar color represents the values are encoded with the same ciphertext.}
\end{figure}
}

%\begin{figure}
%  \myincludegraphics[width=0.6\linewidth]{design_flow}{The design flow of HeroHD}
%\end{figure}


\ignore{
Proposed in \cite{hehdc}, the cosine similarity search of a query hypervector $\vec{\mathcal{H}_q}$ can be modified as a matrix-vector multiplication (MVM) as follows:
\begin{align}
M &= \begin{bmatrix}
  \vec{\mathcal{C}'^1} &
  \vec{\mathcal{C}'^2} &
  \cdots &
  \vec{\mathcal{C}'^L}
\end{bmatrix} \\
\vec{\delta}(\vec{\mathcal{H}_q}, M) &= \vec{\mathcal{H}}_q^\intercal \cdot M
\end{align}
where $\vec{\mathcal{C}'^i}$ is the $i$\textsubscript{th} normalized class hypervector and $L$ is the number of classes.
To optimize the efficiency of MVM operations, previous HE-based PPML works \cite{chou2018faster,lola,mp-fhe-cnn} have introduced several algorithms for packing matrices into HE ciphertext slots. In the case of HE-HDC \cite{hehdc}, the evaluation of the dot product between a query hypervetor and class hypervectors involves homomorphic multiplication followed by a reduction sum.  This reduction sum is achieved through multiple homomorphic rotations and additions, as illustrated in \figref{he-hdc}.

However, sliding window-based object detection using HDC requires cosine similarity search of thousands of query hypervectors for a single image, unlike image classification where only a singe query hypervector is generated. In order to compute multiple query hypervectors simultaneously, HeroHD maps each element of the query hypervectors into a single plaintext, resulting in $D$ plaintext encodings for a single query hypervector. Since each plaintext can pack up to $N$ scalar values, the remaining plaintext slots are used to pack other query hypervectors. A single class hypervector is mapped redundantly into $D$ ciphertexts. \figref{hero-hdc} illustrates the computation of four dot products between four query hypervectors and a single class hypervector. Representing a single element inside a long vector into a single ciphertext allows each element to be computed individually, requiring less amount of homomorphic rotations. However it is usually avoided in most HE-based PPML works since it requires a large size of input batch size to fully utilize the SIMD slots which is not likely in single image classification. We argue that in the case of HE-HDC, the massive amount of query hypervectors generated for a single image can easily fulfill the whole batch size. 

%This allows homomorphic addition and multiplication to be evaluated element-wise, which can be seen as a SIMD operation on vectors. The number of SIMD slots on a single plain/ciphertext is proportional to the degree of the polynomial, usually thousands. Thus, it is crucial to fully exploit parallelism of the ciphertext slots when designing a HE-based program. Previous HE-based PPML that targets image classification with CNN \cite{chou2018faster,lola,mp-fhe-cnn} exploit this parallelism by packing input image pixel values into ciphertext slots \cite{lola} or by packing the channel dimension of CNN weights \cite{mp-fhe-cnn}. HDC based HE inference proposed in \cite{hehdc} fully utilizes the ciphertext slots by packing the hypervector elements inside ciphertext slots. Unlike \cite{hehdc} which takes a single query hypervector as an input, HeroHD targets sliding window-based object detection with HDC where thousands of query hypervectors are generated from a single image. In order to efficiently support a lot of query hypervectors in a single inference, we decide to batch multiple hypervectors 
}

%\subsection{Client-side HE Computation}

%JW: I think this paragraph should be in preliminary or related works section


\ignore{
\begin{table}[t!]
  \caption{Comparison}
  \label{comparison}
  \centering
 % \resizebox{\columnwidth}{!}{
 % think i should remove the number of ct/pt..
  \begin{tabular}{c| c c c c c}
  \toprule
  \multirow{2}{*}{Method} &\multicolumn{2}{c}{Number of}& Message & \multicolumn{2}{c}{Latency (ms)} \\
  \cmidrule{2-3}\cmidrule{5-6} & Ct &  Pt & Size (B) & Enc & Total \\
  \midrule
  Server side HE  &   $D$  &  0  &  32.11M  & 504.12 & 528.27\\
  Client side HE    &   0  &  $D$  &  62.22K   &  38.53 & 61.23\\
  \bottomrule
      \multicolumn{4}{l}{\emph{Note.}~ $k=2$, $D=1024$ and $N=1024$} \\
  \end{tabular}
\end{table}}




\subsection{Optimization 1: HE Scheme-aware Quantization}
\label{subsection_quant}

While HE runtime is mainly determined by $N$ (the polynomial degree of ciphertext), reducing $N$ can negatively impact the arithmetic precision of HE operations. Also HDC's design parameters heavily influence latency and accuracy as illustrated in \figref{dependency}. This suggests that the HE and HDC design parameters must be optimized together globally in order to be effective. 
%We first ?

%\tabref{parameters} summarizes the available modulo size $\log_2 q$ for each polynomial degree $N$, whereas the arithmetic precision $\log_2 t$ should be much lower than $\log_2 q$. 

\begin{figure}
  \myincludegraphics[width=0.8\linewidth]{scheme}{Encryption method comparison between BFV, BGV, and CKKS.}
\end{figure}

\subsubsection{Quantization Opportunity in BGV/BFV}
We find integer HE schemes (BGV/BFV) more suitable for our application for two reasons.  First, they are faster than CKKS when the number of homomorphic multiplications is low \cite{fhebench}. Second, they allow a more tight control of arithmetic precision, which enables further optimization through quantization. 

\figref{scheme} illustrates how message is encrypted into ciphertext in different HE schemes. In CKKS, fixed-point message and noise overlap in the ciphertext where the message can make full use of the $\log_2 q$ bits of precision but the least significant bits may be corrupted due to noise. BGV/BFV scheme reserves for message a certain number of bits (i.e., the plaintext modulo's bit-length $\log_2 t$), leaving the rest of the precision as the noise budget. (Since homomorphic operations gradually increase noise level, the noise budget should be large enough to ensure correct decryption.)
%Therefore, in order to evaluate complicated arithmetic homomorphically, the noise budget should be increased, which can be achieved by either lowering the message precision $\log_2 t$ or increasing the ciphertext polynomial degree.
The noise budget can be increased by either lowering the message precision $\log_2 t$ or increasing $N$ (increasing $N$ increases ciphertext modulo's bit-length $\log_2 q$). %, see \tabref{parameters}).
Since increasing $N$ impacts latency, we seek to reduce message precision to accelerate homomorphic operations without compromising security level.
%The ciphertext modulo's bit-length $\log_2 q$ with respect to $N$ is summarized in \tabref{parameters}.

\subsubsection{BGV/BFV-Aware Quantization}
To maintain the HDC model accuracy at extremely low precision, we apply quantization to both query hypervectors and class hypervectors. One difference between our quantization approach and DNN quantization is that whereas DNN quantization is concerned with reducing multiplication precision only, HE schemes require \textit{every} computation result to be within $\log_2 t$ bits including addition. Thus in order to ensure no overflow happens during addition we introduce a scaling operation after every $g$ HE additions, where $g$ is a design parameter (we use 512). Unlike ciphertext division that is not supported on BGV/BFV, plaintext division can be done only when there exists a modular multiplicative inverse of a divisor for a given plaintext modulo $t$.
Our quantization method bears some similarity with the accumulator scale factor proposed in \cite{azat} where we search for scale factors that has a multiplicative inverse instead of power-of-two values. 

%\jlnote{This is how we actually quantize our HDC model...}

%In order to shorten the latency of HeroHD, we reduce the polynomial degree to the extreme by constraining the arithmetic precision. which is why we choose BFV.\footnote{Our experimental results in \secref{sec:noise_result} indicate that BFV has less noise than BGV.} % We also introduce a zero point in quantization before HE encoding, ensuring every computation is done with unsigned integers.
% Not enough space
%\todonum[]{Some fancy equations explaining quantization}

%\subsection{Flow for Optimizing Design Parameters}

\begin{figure}
  \centering
  \includegraphics[width=0.8\linewidth]{dependency} \\
 \parbox{\linewidth}{\footnotesize  \textit{*Note.~} Increasing $\log_2 t$ does not directly increase noise but reduces the noise \textit{budget}, and hence is similar to increasing noise (or effective noise level).}
  \caption{Relationship among HeroHD parameters.}
  \label{dependency}
\end{figure}

\subsection{Optimization 2: Design Space Exploration for HeroHD}
\label{subsection_design_opt}
\ignore{
\jwnote{make this flowchart shorter or make algorithm}
\begin{figure}
  \myincludegraphics[width=0.5\linewidth]{design_flow}{DSE flow.}
\end{figure}
}

\begin{algorithm} 
\caption{Optimizing [$N$, $\log_2 t$, $D$]}
\label{alg}
\begin{algorithmic}[1]
%\Require $model()$, the unencrypted model
%\Require $N_0$, $\log_2 t_0$, initial HE parameters 
\Procedure{findDmax}{$N$, $\log_2 t$}
\For{1000 times} 
    \State $D_{\max} \leftarrow 1$
    \While{evalHEmodel($N$, $\log_2 t$, $D$) is correct}
        \State $D_{\max} \leftarrow D_{\max}+1$
    \EndWhile
\EndFor%{get average $D_{max}$}
\State \Return  average $D_{\max}$
\EndProcedure

\Procedure{main}{$N_0$}
\State initialize $N \leftarrow N_0$
%\State Initialize $\log_2 t = \log_2 t_0$
\State $\log_2 t$ $\leftarrow$ getMaximumAllowed($N$)
\State $D \leftarrow$ findDmax($N$, $\log_2 t$)
\State $accuracy \leftarrow$ trainHEmodel($N$, $\log_2 t$, $D$)
\While{$\log_2 t \leq$ getMaximumAllowed($N/2$)}
    %\State let $\log_2 t$ be the maximum allowed value for $N$
    \While{$accuracy \geq tol$}
        \State save [$N$, $\log_2 t$, $D$] 
        \State $\log_2 t \leftarrow \log_2 t - 1$
        \State $D \leftarrow$ findDmax($N$, $\log_2 t$)
        \State $accuracy \leftarrow$ trainHEmodel($N$, $\log_2 t$, $D$)
    \EndWhile
    \State $N \leftarrow N/2$
\EndWhile
\State \Return the last saved [$N$, $\log_2 t$, $D$] 
\EndProcedure
\end{algorithmic}
\end{algorithm}

%\jlnote{add one sentence explaining getMaximumAllowed function, and trainHEmodel.}
%Unlike CKKS where message and noise are not clearly distinguished inside a ciphertext, the arithmetic precision in integer HE schemes such as BGV/BFV can be defined exactly as $\log_2 t$ bits. 
%\jwnote{write explanation for algorithm}
Our design space exploration algorithm is presented in \algref{alg}. Whenever the noise level exceeds the noise budget inside a BGV/BGV ciphertext, an overflow happens inside the polynomial coefficients completely destroying the results. Therefore, it is important to know beforehand that the number of HE operations do not exceeds the noise budget for a given $\log_2 t$ and $N$. For a polynomial length $N$ only some specific values of $\log_2 t$ is allowed, getMaximumAllowed() in \algref{alg} returns the availability of $\log_2 t$ for given $N$. The findDmax procedure of \algref{alg} is used to find the maximum $D$ that can be used for every possible combination of $N$ and $\log_2 t$ values. Starting from $N=2^{13}$ and the highest $\log_2 t$ for $N$, we gradually decrease $\log_2 t$ until the HDC model has the highest model accuracy. Note that decreasing $\log_2 t$ will initially benefit the model accuracy by allowing higher $D$, but too low arithmetic precision will decrease the model accuracy. This step is repeated with a lower polynomial size until the lowest $N$ is found with a reasonable model accuracy. 
\ignore{
\begin{table}[]
  \centering
  \caption{Polynomial degree and modulo size }
  \label{parameters}
  \begin{tabular}{ccc}
    \toprule
    Security Level (bits) & $\log_2 N$ & $\log_2 q$ \\
    \midrule
    128 & 10 & 27  \\
    128 & 11 & 54  \\
    128 & 12 & 109 \\
    128 & 13 & 218 \\

    \bottomrule
  \end{tabular}
\end{table}}
\ignore{
\subsection{Design space of HeroHD}
In this section, the design space of HeroHD is listed out and the relationship between them is explained..
\subsubsection{HDC}
\subsubsection{HE Parameters}
\subsubsection{Quantization}
}
\ignore{
\begin{table*}[t]
  \centering
  \caption{Design space parameters for HeroHD}
  \label{terms}
  \begin{tabular}{c|cl}
    \toprule
    Parameter & Symbol & \multicolumn{1}{c}{Meaning} \\
    \midrule
    polynomial degree & $N$ & The degree of ciphertext polynomials, which is same as the number of SIMD slots. Determines the maximum $\log_2 t$. \\
    %\cmidrule{2-3}
    message bit-length & $\log_2 t$ & The number of bits for the message inside the ciphertexts. $\log_2 t$ determins the arithemtic precision. \\
    %\cmidrule{2-3}
     hypervector dimension & $D$ & Dimension of the hypervectors. Larger dimension has better plaintext accuracy but more vulnerable to HE noise. \\
    %\cmidrule{2-3}
    query/class HV precision & QnCm & n-bit quantization for query HVs and m-bit quantization for class HVs. \\   
    %\cmidrule{2-3}
    accumulator scale factor & SF & The scale factor applied before accumulation in order to reduce overflow.\\   
    \bottomrule
  \end{tabular}
\end{table*}}

\begin{table}[t]
  \centering
  \caption{Number of homomorphic operations}
  \label{op_comp}
\begin{tabular}{c|c|ccc}
      \toprule
         & Batch size & \#MulCP             & \#AddCC                   & 
         \#Rot              \\
          \midrule
HE-HDC   & 1          & $k \ceil{\frac{2D}{N}}$ & $k\ceil{\frac{2D}{N}}$ & $\log_2\frac{N}{2}$  \\
HeroHD & $\floor{\frac{N}{k}}$        & $D$   & $D$ & 0           \\ 

%HE-HDC   & 1          & $k\lceil \frac{2D}{N} \rceil$ & $k\lceil \frac{2D}{N} \rceil$ & $\log_2\frac{N}{2}$ & $\lceil \frac{2D}{N} \rceil$ & $k\lceil \frac{2D}{N} \rceil$ \\
%HeroHD & $N$        & $kD$   & $kD$ & 0           & $k$                          & $kD$     \\ 
    \bottomrule
%    \multicolumn{3}{l}{\emph{Note.}~ $k$ is the number of classes.} \\
\end{tabular}
\end{table}

%\subsection{Implementation Detail: Batched HDC Inference Using HE}
\subsection{Efficient HE Representation for Batched HDC Inference}
% I tried to remove this section but couldn't
%\todonum[]{We need to draw a diagram}
\begin{figure}
  \myincludegraphics[width=\linewidth]{batched_he}{Representation of hypervectors and cosine similarity search.}
    %\label{fig_batched-he}
\end{figure}
 %  \jwnote{it is better to have a new diagram comparing HE-HDC and HeroHD and add a legend}
In order to process thousands of query hypervectors generated in HDC-based object detection, HeroHD encodes the elements of query hypervectors into different plaintext polynomials, namely the SIMD representation introduced in \cite{lola}. This allows us to encode $N$ (or $N/2$ for CKKS) vectors at once by utilizing the SIMD slots of an HE scheme, which can be easily fulfilled in HDC-based object detection. 
The cosine similarity operation of HDC on HE can be done as a matrix-vector multiplication as proposed in HE-HDC \cite{hehdc}, whereas in our case, multiple vector dot products are processed simultaneously instead.

Since each query hypervector requires $k$ (the number of classes) cosine similarity operations, a singe query hypervector is encoded into plaintext formats $k$ times redundantly. This result in $\floor{\frac{N}{k}}$ query hypervectors to be computed once as a batched inference. The representation of hypervectors and the HE cosine similarity search is presented in \figref{batched_he}. This encoding has an extra advantage over HE-HDC because it does not require \emph{homomorphic rotation}, reducing the amount of HE noise significantly. \tabref{op_comp} compares the number of HE operations between HE-HDC and HeroHD.



\section{Experiments}
\ignore{
\begin{table}[h]
\centering
\label{hdc_comp}
\caption{Comparison with HDC-based PPML on FACE Dataset}
\begin{tabular}{c|ccccc}
\toprule
\multirow{2}{*}{Method} & Batch & Accuracy & Message  & Latency & \multirow{2}{*}{Throughput} \\
       & Size  & (\%)     & Size (B) & (ms)    &         \\
       \midrule
HE-HDC &  1    &\red{???}&  96.16K & 86.44   &  11.57  \\
HeroHD &  1024 &   100.0   &  31.11K & 143.88  &  7117.04  \\
\bottomrule
\end{tabular}
\end{table}
}
\ignore{
\begin{table*}[h]
  \caption{Comparison with HDC-based PPML on EMOTION Dataset}
  \centering
  \label{table_previous_work}
\begin{tabular}{cc|ccccc}
\toprule
Dataset                  & Method                                             & Batch Size & Accuracy (\%) & Message Size (B) & Latency (s) & Throughtput \\
\midrule
\multirow{4}{*}{FACE \cite{face}}    & CryptoNets~\cite{cryptonets:icml16} & 4096       & 100.0         & 1.92G$^\dagger$            & 294.5         & 16.38       \\
                         & LoLa~\cite{lola}              & 1          & 100.0         & 61.23M$^\dagger$           & 3.62$^\ddagger$        & 0.27$^\ddagger$        \\
                         & HE-HDC \cite{hehdc}                                     & 1          & 99.71         & 96.16K           & 0.094       & 10.63       \\
                         & HeroHD (ours)                                      & 1024        & 100.0         & 31.11K*           & 0.143*       & 7161*        \\
                         \midrule
\multirow{4}{*}{EMOTION \cite{emotion}} & CryptoNets~\cite{cryptonets:icml16}& 4096       & 45.59         & 1.92G$^\dagger$            & ???         & 16.38       \\
                         & LoLa~\cite{lola}             & 1          & 45.59         & 61.23M$^\dagger$           & 3.62$^\ddagger$        & 0.27$^\ddagger$        \\
                         & HE-HDC \cite{hehdc}                                       & 1          & ???           & 96.16K           & 0.094       & 10.63       \\
                         & HeroHD (ours)                                               & 585             & 43.xx                & 128.11K    &0.326     & 1791.61   \\   
                           \bottomrule
                           \multicolumn{5}{l}{\emph{Note.}~ 1. $^\dagger$scaled up according to the sliding window size 64x64.}\\
\multicolumn{5}{l}{~~~~~~~ 2. $^\ddagger$with multithreading enabled.}\\
\multicolumn{5}{l}{~~~~~~~  3. *Our own measurements.}\\
\multicolumn{5}{l}{~~~~~~~  4. \footnote[4]{}Including the hypervector encoding latency.}
\end{tabular}
\end{table*}}

\subsection{Experimental Setup}
To evaluate HeroHD we implemented the HE part of HeroHD using the Pyfhel library \cite{pyfhel}. The HDC model was trained by extending OnlineHD \cite{onlinehd} with a custom quantizer function and HOG. The latency and throughput was measured with a single AMD Ryzen 3970X CPU without multithreading enabled. % To compare the detection accuracy on the FACE dataset \cite{face} with previous HE-based PPML works, the classifier model of CryptoNets \cite{sealcrypto}, LoLa \cite{lola} and HE-HDC \cite{hehdc} was implemented by ourselves, modified to support sliding-window based o detection.

\subsection{HDC Model Accuracy}
\label{subsection_hdc-opt}
%nghao, could you maybe write down the results between OnlineHD, OnlineHD+HOG, FaceHD in terms of encoding latency and accuracy?
%As we mentioned in Section \ref{section_hdod}, the HOG feature extractor can improve the object detection performance regarding accuracy and latency. We use the FACE dataset to show the improvement from the HOG feature extractor. The results are shown in Table \ref{table_hog}. Here we set the window size the same as the image size, and we pass one image each time and calculate the average inference latency. We can observe that the HOG extraction improves around $5\%$ accuracy and $22$ms inference latency.
We evaluated the unencrypted HDC model accuracy of HeroHD on the FACE and EMOTION dataset, both a face detection dataset that can be used for object detection. For a fair comparison with previous PPML works that are crafted to maximize performance on the MNIST dataset, we also present the model accuracy of HeroHD and HE-HDC on the MNIST dataset. Details of the used datasets are summarized in \tabref{table_datasets}.
%To compare the model accuracy with previous HE-based PPML works, we implemented the model structure of CryptoNets \cite{cryptonets:icml16}, LoLa \cite{lola} which shares the same DNN model structure. 
DNN-based approaches, CryptoNets \cite{cryptonets:icml16} and LoLa \cite{lola} were implemented ourselves which shares the same DNN model structure. 
The accuracy of HE-HDC \cite{hehdc} is also compared which uses the HDC classifier proposed in \cite{onlinehd}. \tabref{table_hog} summarizes the model accuracy on the three datasets. Since the FACE dataset is a binary classification dataset, every work except for HE-HDC easily achieves 100\% accuracy. 
By introducing HOG, HeroHD compared to CryptoNets and LoLa has a better accuracy on EMOTION using hypervector dimension $D \geq 4096$.
\begin{table}[t]
  \centering
  \caption{Datasets}
   \label{table_datasets}
\begin{tabular}{c|ccc}
\toprule
                            & Image size                         & \#classes     & Train size                    \\
                            \midrule
FACE     \cite{face}                  & 1024 $\times$ 1024                 & 2                     & 40,172                                     \\
MNIST  \cite{deng2012mnist}                     & 28 $\times$ 28                     & 10                    & 60,000                                      \\
EMOTION \cite{emotion}& 48 $\times$ 48 & 7 & 36,685\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
  \centering
  \caption{Unencrypted Model Accuracy Comparison}
   \label{table_hog}
      \resizebox{\linewidth}{!}{  
\begin{tabular}{cc|ccc}
    \toprule
\multirow{2}{*}{Model}         & & \multicolumn{3}{c}{Accuracy (\%)}\\
                               & D  & \multicolumn{1}{c}{FACE} & MNIST& \multicolumn{1}{c}{EMOTION} \\
                                   \midrule
CryptoNets\cite{cryptonets:icml16} / LoLa \cite{lola}&  & 100.000& \textbf{98.950}& 45.597   \\
            \midrule
\multirow{3}{*}{HE-HDC \cite{hehdc}}        & 1K &           95.375            & 94.110 & 36.528                      \\
                               & 4K & 97.600                    & 96.590 & 39.050                      \\
                               & 8K & 95.825                    & 97.160 & 39.774                      \\
                                       \midrule 
\multirow{3}{*}{HeroHD (ours)} & 1K & 100.000                    & 97.710 & 44.734                      \\
                               & 4K & 100.000                   & 98.390 & \textbf{47.910}                      \\
                               & 8K & 100.000                    & 98.260 & \textbf{48.899}      \\
                                   \bottomrule
\end{tabular}}
\end{table}

%\subsection{Choice of HE Scheme}
%Although CKKS is the most widely used HE scheme in PPML works, the approximate computation of CKKS makes it hard to ensure the correctness of the decrypted results. Furthermore, integer HE schemes such as BGV and BGV are proven to be faster on low multiplicative depth \cite{fhebench}. Therefore, instead of CKKS, we benchmark the noise growth of BGV in BFV for HeroHD to determine the HE scheme. Since longer hypervector dimension $D$ results in more noise, we observe that there is a certain level of 
%Varying $N$ and $\log_2 t$, we evaluated the maximum 


%server-side HE
%client             server
%encCt+dec          computeHE
%encPt+compute      dec

\subsection{Effect of Our Client-Side Approach}
%Although the client-side approach of HeroHD does not affect the cosine similarity search latency, it can drastically reduce the HE encryption overhead. 
To demonstrate the runtime advantage of our client-side approach, we 
compare the traditional server-side HE vs.\ our client-side HE in terms of
client runtime (see \figref{client-side_res_new}). For the client-side approach, the runtime is divided in two parts: the HE compute latency along with the plaintext encoding latency. The server runtime is obviously reduced by our method, and the full runtime results are listed in \tabref{comparison}. 
%, the total HE latency of HeroHD is divided into two parts: the HE compute latency along with the plaintext encoding latency for the client-side approach, and the HE compute latency along with the ciphertext encryption latency for the server-side approach. The results are presented in \figref{client-side_res}. 
\begin{figure}
  \myincludegraphics[width=\linewidth]{client-side_res_new}{Client runtime reduction of client-side HE over server-side HE.}
  %Switch sides, move HE compute (black) to the bottom
\end{figure}
\begin{table}[]
  \caption{Comparison of Client-side HE (HeroHD) and Server-side HE}
  \label{comparison}
  \centering
\begin{tabular}{ccc|cc}
\toprule
\multirow{2}{*}{Method}                  & \multirow{2}{*}{N}        & \multicolumn{1}{c|}{\multirow{2}{*}{D}} & Message  & Total\\  
                                         &                           & \multicolumn{1}{c|}{}                   & Size (B) & Latency (ms)\\ \midrule
\multirow{4}{*}{\shortstack[c]{Client-side HE \\ (HeroHD)}}          & \multirow{2}{*}{$2^{11}$} & 1K                 &          31.1K&                         43.99\\
                                         &                           & 2K                 &   31.1K   &                            87.72\\
                                         & \multirow{2}{*}{$2^{12}$} & 1K                 &      121.1K    &                            105.27\\
                                         &                           & 2K                 &        121.1K &                           204.58\\
                                         \midrule
\multirow{4}{*}{Server-side HE} & \multirow{2}{*}{$2^{11}$} & 1K                 &    31.86M  &                          351.95 ($\times$8.00)\\
                             &                           & 2K                 &            63.71M     &                           702.86 ($\times$8.01)\\
                                         & \multirow{2}{*}{$2^{12}$} & 1K                 &        131.2M  &                           1163.95 ($\times$11.05)\\
                                   &                           & 2K                 &             262.4M   &                      2303.22 ($\times$11.23)\\
                        \bottomrule
\end{tabular}
\end{table}
%\jwnote{Revise explanation} 
The client runtime of HeroHD is dominated by the HE encoding/encryption overhead, where using the client-side approach is faster than server-side approach by $9.1\times$ on average. The total HE runtime, including the server runtime, is improved by $8.1\times$ for $N=2^{11}$ and $11.2\times$ for $N=2^{12}$. Along with the latency improvement, the HE message size that has to be transmitted between the client and the server is also reduced in the client-side approach by $D$ times, which is very significant. 

\begin{figure}
% need to make the figure better..
    \myincludegraphics[width=\linewidth]{noise_growth}{$D_{max}$ for various $N$ and $\log_2 t$. The standard deviation is represented as the width of shaded regions.}
\end{figure}

\subsection{Effect of HE Noise}
\label{sec:noise_result}
Longer hypervector dimension in HeroHD accumulates more HE noise, resulting in incorrect values. To find out $D_{max}$, the maximum $D$ supported for polynomial length $N$ and message bit-length $\log_2 t$, we evaluated random integers on HeroHD and gradually increased the hypervector dimension $D$ until the results were incorrect. Due to the random nature of HE noise, there is no deterministic upper-bound for hypervector dimension. Instead, we repeated the process 1000 times for each parameter settings where the mean average and the standard deviation is presented in \figref{noise_growth}. The result shows a clear trade-off between $\log_2 t$ and $D_{max}$ where decreasing $\log_2 t$ increases $D_{max}$ exponentially. We also observe that the noise management on BFV is better compared to BGV, allowing more HE operations. Driven by this observation, we have only used BFV in the experiments below.
\ignore{
\begin{table}[]
  \centering
    \caption{Latency and Throughput Results for different parameters}
\begin{tabular}{cc|rrr|r}
    \toprule
\multirow{2}{*}{N}    & \multirow{2}{*}{D} & \multicolumn{3}{c}{Latency}   & \multirow{2}{*}{Throughput} \\
                      &                    & HV Encoding & HE Inference & Total  &                             \\
                          \midrule
\multirow{4}{*}{$2^{11}$} & 1K                 & 99.89     &  45.68  &145.57 &7034.38                   \\
                      & 2K                 &137.37     &  90.72  &228.09 &4489.38                \\
                      & 4K                 & 205.04    &  179.81 & 384.85&2660.79         \\
                      & 8K                 &335.96   & 366.84 & 702.80&1457.04                     \\
                      \midrule
\multirow{4}{*}{$2^{12}$} & 1K                 & 197.93   & 104.92&302.85 & 6762.42               \\
                      & 2K                 &257.96   & 210.81 &468.77 &4368.88                    \\
                      & 4K                 & 385.58& 416.23 &801.81&2554.22                \\
                      & 8K                 &624.98& 833.86 & 1458.84&1403.86   \\
                          \bottomrule
\end{tabular}
\end{table}
}
\subsection{Effect of HeroHD Optimizations}
%Unlike CKKS where the noise is overlapped with the message, a single overflow in BFV completely destroys the computation results. 
The unoptimized implementation of HeroHD uses 16-bit quantization for the class and query hypervectors, where HE computation is correct only for polynomial degree $N \geq 2^{13}$. Following the optimization method from \secref{subsection_design_opt}, we have optimized HeroHD for the FACE and EMOTION dataset, whose results are listed in \tabref{opti_results}. For the FACE dataset, quantizing query hypervectors into 6 bits and class hypervectors into 2 bits can reduce the polynomial degree to $N=2^{11}$. In the case of EMOTION dataset, model accuracy of 44.97\% can be reached with $N=2^{11}$. This optimization improves the HE latency by $6.65\times$ for the FACE dataset without any accuracy loss and $9.74\times$ for the EMOTION dataset with minimal accuracy drop. 

\begin{table}[]
\centering
    \caption{Effect of HeroHD Optimization}
    \label{opti_results}
\begin{tabular}{c|cc|cc}
\toprule
                & \multicolumn{2}{c|}{FACE \cite{face}} & \multicolumn{2}{c}{EMOTION \cite{emotion}} \\
                & Initial  & Optimized  & Initial   & Optimized   \\
                \midrule
N               & 8192         & 2048       & 8192          & 2048        \\
$\log_2 t$      & 60           & 17         & 60            & 16          \\
D               & 1024         & 1024       & 8192          & 5632        \\

Q/C*    & 16/16       & 6/2       & 16/16        & 8/8         \\
\midrule
Accuracy (\%)   & 100.00          & 100.00       & 48.899        & 44.970         \\
HE Latency (ms) & 292.69       & \textbf{43.99}      & 2306.47       & \textbf{236.85}     \\
 \bottomrule
 \multicolumn{5}{l}{*Q-bit quantization for query HVs and C-bit quantization for class HVs.}\\
\end{tabular}
\end{table}

%the old version
\subsection{Comparison with Other HE-based PPML}

\begin{table}[h]
  \caption{Comparison with Previous PPML works}
    \centering
  \label{table_previous_work} 
   \resizebox{\linewidth}{!}{  
\begin{tabular}{c|cc|ccc}
\toprule
Dataset          &\multicolumn{2}{c|}{FACE} & \multicolumn{3}{c}{EMOTION}  \\
Method   & HE-HDC    & HeroHD   & CryptoNets & LoLa & HeroHD \\ 
\midrule
Batch Size       &     1     &  1024      &    4096*      &  1*   & 292    \\
Accuracy (\%)    & 97.23  &   100.0    & 45.59        &  45.59 & 44.97     \\
Message Size (B) &    96.2K  &   \textbf{31.1K}  &    1.92G & 61.2M  & \textbf{31.1K}    \\
Latency (s)      &    \textbf{0.086}  &   0.144  &    250*    & 2.2*$^\dagger$   &\textbf{0.317}    \\
Throughput       & 11.57  &\textbf{7117.04}   &  16.38*    & 0.45*$^\dagger$    & \textbf{912.13}        \\

\bottomrule
\multicolumn{5}{l}{*Quoted from original paper. ~$^\dagger$With multithreading enabled.}
\end{tabular}}
\end{table}
\ignore{
\begin{table}[h]
  \caption{Comparison with Previous PPML works}
  \centering
  
  \label{table_previous_work} 
\begin{tabular}{cc|ccccc}
\toprule
\multirow{2}{*}{DS} & \multirow{2}{*}{Method} & Batch & Accuracy & Message  & Latency & \multirow{2}{*}{Throughput} \\
     &  & Size  & (\%)     & Size (B) & (s)    &         \\
              \midrule
\multirow{2}{*}{F} & HE-HDC* &  1    &97.23&  96.16K & \textbf{0.086}   &  11.57  \\
& HeroHD* &  1024 &   100.0   &  \textbf{31.11K} & 0.144  &  \textbf{7117.04}  \\
       
       \midrule
\multirow{3}{*}{E} & CryptoNets& 4096       & 45.59         & 1.92G    & 250         & 16.38   \\
& LoLa            & 1          & 45.59  & 61.23M   & 2.2$^\dagger$   & 0.45$^\dagger$        \\
& HeroHD    & 292             & 44.97   & 31.11K    &\textbf{0.317}     & \textbf{912.13}   \\ 
\bottomrule
\multicolumn{5}{l}{*Results on the FACE dataset.}\\
\multicolumn{5}{l}{$^\dagger$With multithreading enabled.}
\end{tabular}
\end{table}}

\ignore{
% why not MNIST?
\subsection{Comparison with Other HE-based PPML}
\begin{table}[h]
  \caption{FACE Performance Comparison}
  \centering
  \label{table_previous_work}
\begin{tabular}{c|ccccc}
\toprule
\multirow{2}{*}{Method} & Batch & Accuracy & Message  & Compute & Throughput \\
       & size  & (\%)     & size (B) & latency (s)    & (frames/s)        \\
              \midrule

       %\midrule
 CryptoNets& 4096       & 100.0      & 1.92G    & 250         & 16.38   \\
 LoLa            & 1          & 100.0  & 61.23M   & 2.2$^\dagger$   & 0.45$^\dagger$  \\
 HE-HDC* &  1    &97.23&  96.16K & \textbf{0.086}   &  11.57  \\
HeroHD* &  1024 &   100.0   &  31.11K & 0.144  &  \textbf{7117.04}  \\
    
%HeroHD    & 292             & 44.97   & 31.11K    &\textbf{0.317}     & \textbf{912.13}   \\ 
\bottomrule
\multicolumn{5}{l}{*Measurement from original papers.}\\
\multicolumn{5}{l}{$^\dagger$With multithreading enabled.}
\end{tabular}
\end{table}



\begin{table}[h]
  \caption{EMOTION Performance Comparison}
  \centering
  \label{table_previous_work}
\begin{tabular}{c|ccccc}
\toprule
\multirow{2}{*}{Method} & Batch & Accuracy & Message  & Compute & Throughput \\
       & size  & (\%)     & size (B) & latency (s)    & (frames/s)        \\
              \midrule

       %\midrule
 CryptoNets& 4096       & 45.59         & 1.92G    & 250         & 16.38   \\
 LoLa            & 1          & 45.59  & 61.23M   & 2.2$^\dagger$   & 0.45$^\dagger$  \\
 HE-HDC* &  1    &39.77&  96.16K & \textbf{0.086}   &  11.57  \\
HeroHD* &  292 &   44.97   &  31.11K & 0.317  &  \textbf{912.13}  \\
    
%HeroHD    & 292             & 44.97   & 31.11K    &\textbf{0.317}     & \textbf{912.13}   \\ 
\bottomrule
\multicolumn{5}{l}{*Results on the FACE dataset.}\\
\multicolumn{5}{l}{$^\dagger$With multithreading enabled.}
\end{tabular}
\end{table}
}

HeroHD is compared with HE-HDC \cite{hehdc} using the FACE dataset and DNN-based PPML methods CryptoNets \cite{cryptonets:icml16} and LoLa \cite{lola} with the EMOTION dataset. We implemented HE-HDC by ourselves where the HDC classifier was modified to have two class hypervectors for the FACE dataset.  
%HeroHD is compared with previous HE-based PPML methods CryptoNets \cite{sealcrypto}, LoLa \cite{lola} and HE-HDC \cite{hehdc} in terms of detection accuracy, latency, throughput and ciphertext message size with two dataset FACE \cite{face} and EMOTION \cite{emotion}, presented in \tabref{table_previous_work}.
For DNN-based methods CryptoNets and LoLa which are originally designed for the MNIST dataset, the message size is scaled up to match the sliding window size 64x64 and the accuracy of the unencrypted model is presented. The overall result is summarized in \tabref{table_previous_work}. The throughput is calculated as the batch size divided by the latency, which is the number of sliding windows that can be processed in a second. The batch size is determined by the representation of messages into ciphertexts, which cannot be changed. Our results demonstrate that only HeroHD has high enough throughput and short enough inference latency (236.85~ms) that is suitable for real-time object detection. Compared to HE-HDC, HeroHD has a longer latency, mainly because of the HOG feature extraction, which increases the HV encoding latency. However, HeroHD performs batch processing, with superior throughput (612$\times$) than HE-HDC when an input contains many patches as in object detection, as well as having superior accuracy. Compared to DNN-based methods HeroHD has $55.7\sim2027\times$ higher throughput with $6.94\sim787\times$ shorter latency.% DNN-based methods, CryptoNets and LoLa shares the same model structure however has a different ciphertext representation of inputs and model weights. 
% 612 = 0.086 * 1024 / 0.144

\ignore{
- Cases:
CryptoNets
LoLa
LoLa-sliding window (our modification)
HE-HDC
Hero

- FoMs:
Latency
Accuracy
Message size}

\ignore{
\begin{table*}[t!]
\todonum[]{split this in two, I didn't fill in the numbers yet}
  \caption{Comparison with Previous Work}
  \label{table_previous_work}
  \centering
 % \resizebox{\columnwidth}{!}{
  \begin{tabular}{c| c c c c c c}
  \toprule
  \multirow{2}{*}{Method} & Accuracy & Message & \multirow{2}{*}{Throughput}&
  \multicolumn{3}{c}{Latency (s)} \\
  \cmidrule{5-7}
  &  (\%) & Size (B)  && HD Encoding & Encryption & Inference \\
  \midrule
  CryptoNets~\cite{cryptonets:icml16}  &   98.95  &  367.5M$^\dagger$  & 13.9 &   & 44.5$^\dagger$  &  250$^\dagger$ \\
  LoLa~\cite{lola}         &   98.95  &  11.72M*  &  0.27 && 1.42*  &  2.2 $\ddagger$ \\
  LoLa-Small~\cite{lola}      &   96.92  &  11.72M*  &  0.58 &&  1.42*  &  0.29 $\ddagger$\\
  HE-HDC \cite{hehdc}  &   97.10*  &  96.16K*  &   10.6& ?? & 0.011*\footnote[4]{} &  0.083* \\
 HeroHD (ours)  &   97.10*  &  96.16K*  &    ~5000 &  0.083* & &\\
  \bottomrule
\multicolumn{5}{l}{\emph{Note.}~ 1. $^\dagger$for a batch size of 4096 (other works use the batch size of 1).}\\
\multicolumn{5}{l}{~~~~~~~ 2. $^\ddagger$with multithreading enabled.}\\
\multicolumn{5}{l}{~~~~~~~  3. *Our own measurements.}\\
\multicolumn{5}{l}{~~~~~~~  4. \footnote[4]{}Including the hypervector encoding latency.}
  \end{tabular}
\end{table*}
}
\ignore{
\begin{table}[h]
  \caption{Comparison of Client-side HE (HeroHD) and Server-side HE}
  \label{comparison}
  \centering
 % \resizebox{\columnwidth}{!}{
 % think i should remove the number of ct/pt..
  \begin{tabular}{c| c c c}
  \toprule
  \multirow{2}{*}{Method} & Message & \multicolumn{2}{c}{Latency (ms)} \\
  \cmidrule{3-4}& Size (B) & Encrption & Total \\
  \midrule
  Server-side HE  &   32.14M  & 504.12 & 528.27\\
  Client-side HE (HeroHD)   &    32.11K   &   27.76& 45.68\\
  \bottomrule
      \multicolumn{4}{l}{\emph{Note.}~ $k=2$, $D=1024$ and $N=2048$} \\
  \end{tabular}
\end{table}
}

\section{Conclusion}
We presented HeroHD, an improved HDC-based PPML that can achieve real-time object detection on BFV. Our novel features include (i) client-side HE which reduces the encryption overhead by $9.1\times$ (ii) BFV/BGV-aware quantization and (iii) a novel parameter optimization method that improves HE latency by $6.65\sim 9.74\times$. Our results clearly demonstrate that HeroHD can outperform state-of-the-arts PPML methods with $55.7\sim2027\times$ higher throughput and $6.94\sim787\times$ shorter latency.
%\cite{nttpim}

